Learning with Local Gradients at the Edge

To enable learning on edge devices with fast convergence and low memory, we present a novel backpropagation-free optimization algorithm dubbed Target Projection Stochastic Gradient Descent (tpSGD). tpSGD generalizes direct random target projection to work with arbitrary loss functions and extends target projection for training recurrent neural networks (RNNs) in addition to feedforward networks. tpSGD uses layer-wise stochastic gradient descent (SGD) and local targets generated via random projections of the labels to train the network layer-by-layer with only forward passes. tpSGD doesn't require retaining gradients during optimization, greatly reducing memory allocation compared to SGD backpropagation (BP) methods that require multiple instances of the entire neural network weights, input/output, and intermediate results. Our method performs comparably to BP gradient-descent within 5% accuracy on relatively shallow networks of fully connected layers, convolutional layers, and recurrent layers. tpSGD also outperforms other state-of-the-art gradient-free algorithms in shallow models consisting of multi-layer perceptrons, convolutional neural networks (CNNs), and RNNs with competitive accuracy and less memory and time. We evaluate the performance of tpSGD in training deep neural networks (e.g. VGG) and extend the approach to multi-layer RNNs. These experiments highlight new research directions related to optimized layer-based adaptor training for domain-shift using tpSGD at the edge.

==> connections.tex <==
\subsection{Connections to Existing Projection-Based Training Algorithms}

\begin{table*}
  \centering
  \begin{tabular}{|c|c|l|}
    \hline
     Method & $J_{i}(.)$ & \multicolumn{1}{|c|}{$w_{i}^{(t+1)}$} \\ \hline
     DFA & Cross-Entropy(y^{*}, y_{K}) & $w_{i}^{(t)} + \eta B_{i}(y^{*} - y_{K})\odot\sigma'_{i}(z_{i})$  \\
     sDFA & Cross-Entropy(y^{*}, y_{K}) & $w_{i}^{(t)} + \eta B_{i}\text{sign}(y^{*} - y_{K})\odot\sigma'_{i}(z_{i})$ \\
     DRTP & Cross-Entropy(y^{*}, y_{K}) & $w_{i}^{(t)} + \eta B_{i}y^{*}\odot\sigma'_{i}(z_{i})$ \\
     tpSGD\_{$\ell1$} & $||B_{i}y^{*} - y_{i}||_{1}$  & $w_{i}^{(t)} + \eta \text{sign}(B_{i}y^{*} - y_{i})\odot\sigma'_{i}(z_{i})$ \\
     tpSGD\_{$\ell2$} & $||B_{i}y^{*} - y_{i}||_{2}^{2}$ & $w_{i}^{(t)} + \eta (B_{i}y^{*} - y_{i})\odot\sigma'_{i}(z_{i})$ \\
    \hline
  \end{tabular}
    \caption{We show the relation between various projection-based methods for training neural networks. In particular, we look at the loss functions $J_{i}(.)$ that each approach is attempting to minimize as well as the weight update $w_{i}^{(t+1)}$ at layer $i$ for iteration $t+1$. Note that we incorporate multiplicative constants into $\eta$.}\label{tab:connections}
\end{table*}

tpSGD shares close connections with a few prominent BP-free, projection-based training algorithms. In some cases, tpSGD acts as a generalization. We highlight connections between Direct Feedback Alignment (DFA) \cite{nokland2016direct}, Error-Sign-Based Direct Feedback Alignment (sDFA) \cite{Frenkel_2021}, Direct Random Target Projection (DRTP) \cite{Frenkel_2021}, and our novel tpSGD approach (tpSGD using layer-wise $\ell1$-error (tpSGD\_{$\ell1$}) and $\ell2$-error (tpSGD\_{$\ell2$})).

Consider the case of a simple linear layer $i$ with non-linear activation function: $y_i = \sigma_{i}(z_i)=\sigma_{i}(x_iW_i)$. We define the following quantities, $J(.)$ is a loss function, $x_i$ is the input of layer $i$, $y_i$ is the output of layer $i$, $W_{i}$ are the weights associated with layer $i$, $\sigma_{i}(.)$ is the non-linear activation function associated with layer $i$, $\delta y_{i}$ is the estimated loss gradients for the outputs of layer $i$, $y_K$ is the predicted output of the final layer, $y^{*}$ is the ground truth one-hot encoding of the labels, $\sigma_{i}'(.)$ is derivative of the non-linear activation function of layer $i$, $B_{i}$ is the layer-dependent projection matrix of the targets for layer $i$, and $\eta$ is the learning rate.

In Table \ref{tab:connections}, we inspect the optimization objectives of the aforementioned algorithms and investigate how this affects the weight update steps at layer $i$. The layer-wise weight update rules are  similar to one another, but each algorithm has subtle distinctions in their assumptions, leading to different optimization behaviors and flexibility in the types of training pipelines they are compatible with. 

DFA, sDFA, and DRTP all attempt to minimize a global objective (cross-entropy between the ground truth labels and final layer output) using noisy gradient steps. DFA and sDFA require a complete forward pass through the network. Then these approaches compute estimated loss gradients for a given layer based on random projections of the gradients of the loss at the final layer. sDFA uses only the sign of the loss gradients whereas DFA uses the full magnitude of the loss gradients. Since both of the methods require a full pass through the network, they are not compatible with tpSGD.

DRTP makes use of the fact that labels are one-hot encodings to simplify sDFA, where DRTP's loss gradients are a surrogate of those of sDFA with shift and rescaling operations applied. Following the reasoning of Frenkel et al. \cite{Frenkel_2021}, we look at the behavior of $e_{sdfa} = sign(y^{*}-y_{K})$ when $y^{*}_{c}$ is 1 and when $y^{*}_{c}$ is 0. We assume $y^{*}_{c} \in \{0,1\}$ (i.e., the ground truth label for a given class is exactly zero or one) and $y_{K}_{c} \in (0,1)$ (i.e., the prediction of the final layer for a given class is in the range zero or one, non-inclusive). Under this assumption, $y^{*}_{c}$ never exactly equals $y_{K_c}$ (i.e., there is always some prediction error). The loss gradient for sDFA can be expressed as:
$$
e_{sdfa_c} = \text{sign}(y^{*}_{c}-y_{K_c}) =
\begin{cases}
1 & \text{if} \; c=c^{*} \\
-1 & \text{otherwise}
\end{cases} \\
,y^{*}_{c} \neq y_{K_c}
$$
$c$ is the index of the one-hot vector and $c^{*}$ is the true class.

The key observation here is that $e_{sdfa_c}$ will always be $+1$ when $y^{*}=1$, and it will always be $-1$ when $y^{*}=0$, regardless of the values of the prediction $y_{K}$, effectively decoupling the estimated loss gradients from the final layer predictions. The loss gradient associated with DRTP is simply a scaling and shifting of $e_{sdfa_c}$ under the above assumptions:
$$
e_{drtp_c} = \frac{1 + \text{sign}(y^{*}_{c}-y_{K_c})}{2} =
\begin{cases}
1 & \text{if} \; c=c^{*} \\
0 & \text{otherwise}
\end{cases} \\
,y^{*}_{c} \neq y_{K_c}
$$
Note $e_{drtp} = y^{*}$, meaning the one-hot labels can serve as the estimated gradient of the loss. To obtain layer-wise gradients w.r.t. the global loss, DRTP uses a random projection matrix to project these one-hot labels as the estimated loss gradients for the global objective. Frenkel et al. showed that for networks consisting of an arbitrary number of linear layers followed by a non-linear activation with cross-entropy as the loss function, DRTP produces estimated gradients within $90^{\circ}$ of the BP gradients, leading to learning, and they experimentally validated that DRTP works with less constrained feedforward architectures. DRTP does not require a full forward pass before updating the weights (no update locking), and DRTP can update layers independent of one another (no issues with weight transport), making DRTP fully compatible with tpSGD. Different layers in the same network can be optimized via either tpSGD or DRTP without issue. In the rest of the paper, we regard DRTP as a subset of the capabilities provided by tpSGD. When DRTP is mentioned, we specifically refer to the aforementioned variations of cost functions and weight updates.   

Finally, we consider our novel tpSGD-style learning. In contrast to other approaches, tpSGD tries to minimize a collection of local losses, with the intention of learning representations that promote reduction of the global loss. tpSGD locally optimizes layers, forcing the layer outputs to align with random projections of the one-hot ground truth labels (serving as layer-wise targets for optimization). tpSGD tries to learn representations such that instances from the same class are well-separated from instances of other classes within the same layer, and representations from two different layers should be well-separated from one another. tpSGD is compatible with any generic layer-wise loss between the layer-wise targets and layer-wise outputs, but we explicitly consider the $\ell1$-norm and $\ell2$-norm for this paper.

%The layer-wise weight update rules are  similar to one another, but each algorithm has subtle distinctions in their assumptions, leading to different optimization behaviors and flexibility in the types of training pipelines they are compatible with. %tpSGD is especially well-suited for cases requiring low-memory compute, such as optimizing models on edge computing hardware.


% tpSGD can be thought of as a generalization of DRTP. In order to understand the differences between tpSGD and DRTP, we first look at how DRTP projects an error signal to a layer. DRTP is a simplified version of error-sign-based direct feedback alignment (sDFA). If we assume targets $y^*$ are binary one-hot encodings of class labels, then sDFA randomly projects the sign of the error ($e = y^* - y_{K}$) at the final layer $K$, e.g., the gradients w.r.t. the target at layer $k$ can be expressed as $\delta y_{k}^{dfa} = B_{k}e$. Instead, DRTP projects the targets themselves \texit{as the error signal}: $\delta y_{k}^{drtp} = B_{k}y^*$. Using the targets  $y^*$ as the error signal acts a surrogate for the error sign vector used in sDFA, where shift and rescaling operations are applied to $sign(e)$: 
% $$y_c^{*} = \frac{1 + sign(e_c)}{2} =
% \begin{cases}
% 1 & \text{if} \; c=c^{*} \\
% 0 & \text{otherwise}
% \end{cases} 
% $$
% where $c$ is the $c^{th}$ element of a one-hot vector of length $C$ (number of classes). Note that this assumes the special case where the error is never exactly zero.

% In contrast, tpSGD is not tied to a particular error signal, but instead uses an error that tries to bring the output of each layer $y_k$ closer to a random projection of the targets to that layer $B_{k}y^{*}$. In this work, for the cases of linear and convolutional layers, we set the error associated with tpSGD to be the mean-squared error (MSE) between the projected target and the output of layer $k$: $e^{tpSGD\_MSE} = ||B_{k}y^{*} - y_{k}||^{2}_{2}, \delta y_{k}^{tpSGD\_MSE} = 2(B_{k}y^{*} - y_{k})$. 

% If we look at the update equations of a linear layer between tpSGD and DRPT for a set of weights $w_k$ at layer $k$, we note they are very similar but capture slightly different information:
% \begin{align}
% tpSGD\_MSE:\; & w_{k}^{t+1} = w_{k}^{t} + \eta (B_{k}y^{*} - y_{k} &&) \odot y_{k}', \\ 
% DRTP: \; & w_{k}^{t+1} = w_{k}^{t} + \eta (B_{k}y^{*} &&) \odot y_{k}'
% \end{align} 
% where $\eta$ is the learning rate and $\odot$ is elementwise multiplication and the ``2'' from $\delta y_{k}^{tpSGD\_MSE}$ is incorporated into $\eta$.

% In the case of the recurrent layers, we actually use the error projected by DRTP, but since tpSGD assumes independence between layers, this is still compatible with the rest of the network layers which are optimized via tpSGD.

